Optimal QoS-Aware Network Slicing for Service-Oriented Networks with Flexible Routing

In this paper, we consider the network slicing problem which attempts to map multiple customized virtual network requests (also called services) to a common shared network infrastructure and allocate network resources to meet diverse quality of service (QoS) requirements. We first propose a mixed integer nonlinear program (MINLP) formulation for this problem that optimizes the network resource consumption while jointly considers QoS requirements, flow routing, and resource budget constraints. In particular, the proposed formulation is able to flexibly route the traffic flow of the services on multiple paths and provide end-to-end (E2E) delay and reliability guarantees for all services. Due to the intrinsic nonlinearity, the MINLP formulation is computationally difficult to solve. To overcome this difficulty, we then propose a mixed integer linear program (MILP) formulation and show that the two formulations and their continuous relaxations are equivalent. Different from the continuous relaxation of the MINLP formulation which is a nonconvex nonlinear programming problem, the continuous relaxation of the MILP formulation is a polynomial time solvable linear programming problem, which makes the MILP formulation much more computationally solvable. Numerical results demonstrate the effectiveness and efficiency of the proposed formulations over existing ones.

==> section_conclusion.tex <==
\section{Conclusions}
\label{sect:conclusion}
In this paper, we have investigated the network slicing problem that plays a crucial role in 5G and B5G networks and  proposed a new MILP formulation.
The proposed formulation minimizes a weight sum the total power consumption and the total link  capacity consumption of the whole network  subject to the E2E delay and E2E reliability constraints of all services and the capacity constraints of all cloud nodes and links. 
Numerical results demonstrate the effectiveness  and efficiency of the proposed formulation. 
More specifically, compared with those in \cite{Vizarreta2017,Chen2021b}, our proposed formulation is much more effective in terms of fully exploiting the flexibility of traffic routing and guaranteeing the E2E reliability of all services; compared with those in \cite{Promwongsa2020}, our proposed formulation is much more computationally solvable.
In addition, our analysis shows the importance of incorporating the total link capacity consumption term into the objective function of the network slicing problem. 
